Predicting UAV Type: An Exploration of Sampling and Data Augmentation for Time Series Classification

Unmanned aerial vehicles are becoming common and have many productive uses. However, their increased prevalence raises safety concerns -- how can we protect restricted airspace? Knowing the type of unmanned aerial vehicle can go a long way in determining any potential risks it carries. For instance, fixed-wing craft can carry more weight over longer distances, thus potentially posing a more significant threat. This paper presents a machine learning model for classifying unmanned aerial vehicles as quadrotor, hexarotor, or fixed-wing. Our approach effectively applies a Long-Short Term Memory (LSTM) neural network for the purpose of time series classification. We performed experiments to test the effects of changing the timestamp sampling method and addressing the imbalance in the class distribution. Through these experiments, we identified the top-performing sampling and class imbalance fixing methods. Averaging the macro f-scores across 10 folds of data, we found that the majority quadrotor class was predicted well (98.16%), and, despite an extreme class imbalance, the model could also predicted a majority of fixed-wing flights correctly (73.15%). Hexarotor instances were often misclassified as quadrotors due to the similarity of multirotors in general (42.15%). However, results remained relatively stable across certain methods, which prompted us to analyze and report on their tradeoffs. The supplemental material for this paper, including the code and data for running all the experiments and generating the results tables, is available at https://osf.io/mnsgk/.

==> Tables/classDistTrainTest.tex <==
\begin{table*}[!htb]\centering
\begin{threeparttable}[!htb]\centering
\scriptsize
\begin{tabular}{lrrrrr@{\hspace{0.6cm}}rrrr@{\hspace{0.6cm}}rrrrr}\toprule
& &\multicolumn{4}{c}{Quadrotor} &\multicolumn{4}{c}{Fixed-Wing} &\multicolumn{4}{c}{Hexarotor} \\\midrule
& &Train &Test Fold &Train Class &Test Class &Train &Test Fold &Train Class &Test Class &Train &Test Fold &Train Class &Test Class \\ & &Count &Count &\%  &\% &Count &Count &\% &\% &Count &Count &\% &\% \\
\arrayrulecolor{gray}\hline
No Changes & &11592 &1288 &94.17\cellcolor{blue1} &94.43 &378 &42 &3.07 \cellcolor{green4} &3.08 &306 &34 &2.49 \cellcolor{purp4} &2.49 \\
\hline
Minority Class &150 &11592 &1288 &91.87 \cellcolor{blue2} &94.43 &567 &42 &4.49 \cellcolor{green3} &3.08 &459 &34 &3.64 \cellcolor{purp3} &2.49 \\ Increase
&200 &11592 &1288 &89.44 \cellcolor{blue3} &94.43 &756 &42 &5.83 \cellcolor{green2} &3.08 &612 &34 &4.72 \cellcolor{purp2} &2.49 \\
&250 &11592 &1288 &87.12 \cellcolor{blue4} &94.43 &949 &42 &7.13 \cellcolor{green1} &3.08 &765 &34 &5.75 \cellcolor{purp1} &2.49 \\
\hline
Majority Class &25 &8694 &1288 &92.71 \cellcolor{blue2} &94.43 &378 &42 &4.03 \cellcolor{green3} &3.08 &306 &34 &3.26 \cellcolor{purp3} &2.49  \\ Decrease
&50 &5796 &1288 &89.44 \cellcolor{blue3} &94.43 &378 &42 &5.83 \cellcolor{green2} &3.08 &306 &34 &4.72 \cellcolor{purp2} &2.49 \\
&75 &2898 &1288 &80.9 \cellcolor{blue4} &94.43 &378 &42 &10.55 \cellcolor{green1} &3.08 &306 &34 &8.54 \cellcolor{purp1} &2.49 \\
\bottomrule
\end{tabular}
    \begin{tablenotes}
        \item Color gradient- Class Contribution Increases and Decreases
    \end{tablenotes}

\smallskip

\caption{Class Distributions in Train and Test: The class distributions for the quadrotor, fixed-wing and hexarotor classes alongside their changes as we incorporate more instances for the minority class and remove instances from the majority class. The number of train instances decrease or increase accordingly (darker indicates more instances), but the number of test instances remain the same and are unchanged to maintain consistency for the unseen examples. We keep this consistency in the test instances so that there is no additional bias introduced by the augmented or decreased samples.}
\label{tab:ClassDistributionTrainTest}

\end{threeparttable}
\end{table*}



==> Tables/classDistribution.tex <==
\begin{table*}[!htb]\centering
\begin{threeparttable}[!htb]\centering
\scriptsize
\begin{tabular}{lrrrrrrrr}\toprule
&Features &Quad Count &Fixed Count &Hex Count &Quad Data \%  &Fixed Data \% &Hex Data \% \\ \midrule 
Base Feats &'vehicle\_local\_position \textbar x', \\
(From Paper) &'vehicle\_local\_position \textbar y', \\
&'vehicle\_local\_position \textbar y', \\
&'vehicle\_local\_position \textbar z', \\ 
&'vehicle\_attitude\_setpoint \textbar roll\_body', \\
&'vehicle\_attitude\_setpoint \textbar pitch\_body', \\
&'vehicle\_attitude\_setpoint \textbar yaw\_body' &26572 &1320 &1303 &91.02 &4.52 &4.46 \\
\hline
Additional Feats &Base Feats + \\
(From Paper) &‘manual\_control\_setpoint \textbar z’, \\
&‘vehicle\_gps\_position \textbar alt’, \\
&‘battery\_status \textbar temperature’ &12880 &420 &340 &94.43 &3.08 &2.49 \\
\hline
Feat subset 0 &Base Feats + \\
&'vehicle\_gps\_position \textbar epv', \\
&'vehicle\_local\_position \textbar dist\_bottom', \\
&'manual\_control\_setpoint \textbar return\_switch', \\
&'manual\_control\_setpoint \textbar rattitude\_switch', \\
&'vehicle\_local\_position \textbar xy\_reset\_counter', &20670 &754 &709 &93.39 &3.41 &3.2 \\
\hline
Feat subset 1 &Base Feats + \\
&'vehicle\_local\_position \textbar az', \\
&'vehicle\_gps\_position \textbar hdop', \\
&'vehicle\_local\_position \textbar ax', \\
&'vehicle\_gps\_position \textbar eph', \\
&'vehicle\_gps\_position \textbar vdop' &23516 &1005 &952 &92.32 &3.95 &3.74 \\
\hline
Feat subset 2 &Base Feats + \\
&'manual\_control\_setpoint \textbar stab\_switch',\\
&'vehicle\_local\_position \textbar vxy\_max', \\
&'home\_position \textbar valid\_alt', \\
&'vehicle\_gps\_position \textbar lon', \\
&'home\_position \textbar lon' &14573 &1488 &415 &88.45 &9.03 &2.52 \\
\bottomrule
\end{tabular}

\smallskip




\end{threeparttable}

\caption{Class Distributions from Feature Selection Experiment:
The features tested during the feature selection process along with the number of instances per class for each subset. A base set of features are used and added on to each selected subset and compared against the features mentioned in \cite{thresholding}. The distribution of classes remain relatively the same; however, the number of majority instances increases greatly.}


\label{tab:ClassDistributionFeature}

\end{table*}

